Phase transition in the knapsack problem

We examine the phase transition phenomenon for the Knapsack problem from both a computational and a human perspective. We first provide, via an empirical and a theoretical analysis, a characterization of the phenomenon in terms of two instance properties; normalised capacity and normalised profit. Then, we show evidence that average time spent by human decision makers in solving an instance peaks near the phase transition. Given the ubiquity of the Knapsack problem in every-day life, a better understanding of its structure can improve our understanding not only of computational techniques but also of human behavior, including the use and development of heuristics and occurrence of biases.

==> formal-analysis.tex <==
\section{Probabilistic analysis}\label{sec:formal}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Let $N_C$ denote the set of nodes of a knapsack instance that satisfy the capacity constraint and let $N_P$ denote the set of nodes that satisfy the profit constraint.
%%
%A solution to the instance exists \emph{if and only if} $N_C\cap N_P \neq \emptyset$.

%%
In this section, we identify an instance parameter and an \emph{upper bound} for its critical value around which this intersection changes from empty to non-empty (over random instances). 
%Briefly, Markov's inequality implies $\prob{X\!>\!0}\leq \ept[X]$, that is, probability of $X\geq 1$, where $X$ is a non-negative random variable, is bounded by its expectation. 
Let $X$ denote the number of solutions in an instance and calculate the conditions under which its expectation is $0$ (that is, the instances are expected to be unsolvable).

In order to analyse the effect of capacity and profit across random instances, we need to adjust their values to a common scale.
%
Normalisation is one such approach that allows comparing different variables to each other.
%
In our case, we \emph{normalise} capacity and profit of an instance as follows. Given a tuple of positive integers $\tuple{x_1,\ldots,x_n}$ and a real number $y \in [0,\sum_{i=1}^{n}x_i]$, we define a function $\sigma(y, \tuple{x_1,\ldots,x_n})$ that returns the normalised value of $y$ with respect to $\tuple{x_1,\ldots,x_n}$  as:
%%
\begin{equation*}\label{eq:norm}
  \sigma(y,\tuple{x_1,\ldots,x_n}) = \frac{y}{\sum_{i=1}^{n}x_i}.
\end{equation*}


Normalisation of constraints plays an essential role in two key aspects.
%
First, it allows studying the tension between the capacity and the profit constraints. Second, we can analyse their effects across random instances in a systematic way.

Given a knapsack instance with items $I = \set{1,\ldots,n}$ having weights $\tuple{w_1,\ldots,w_n}$, values $\tuple{v_1,\ldots,v_n}$, capacity constraint $c$ and profit constraint $p$, we denote the normalized capacity constraint by $\hat{c}=\sigma(c, \tuple{w_1,\ldots,w_n})$ and the normalized profit constraint by $\hat{p}=\sigma(p, \tuple{v_1,\ldots,v_n})$.
%
A set of items $S\subseteq I$ is a \emph{solution} to an instance if the normalized sum of item weights in $S$ is at most the normalized capacity and the normalized sum of item values in $S$ is at least the normalized profit, or $\sigma(\sum_{i\in S}^{}w_i, \tuple{w_1,\ldots,w_n}) \leq \hat{c}$ and $\sigma(\sum_{i\in S}^{}v_i, \tuple{v_1, \ldots, v_n}) \geq \hat{p}$.
%
In the following we use this as our canonical definition of a knapsack instance. % and a solution.


%In this work, we characterize a phase transition in random knapsack instances.
%
 To characterize a phase transition in random knapsack instances, we assume that weights and values of the items are drawn from the same probability distribution (e.g., uniform) on a set of positive integers $R$. 
 %In addition, we allow for replacements  in the sampling of weights and values.
%
Let $\M(n,R,\hat{c},\hat{p})$ denote such a model representing all instances with $n$ items, whose weights and values are drawn from $R$, with normalised capacity constraint $\hat{c}$ and normalised profit constraint $\hat{p}$.
%

Next, we present the main result of this section:
%
\begin{quote}
\noindent
 \emph{The phase transition for random knapsack instances in $\M(n,R,\hat{c},\hat{p})$ is expected around $\hat{c}/\hat{p}=1$}.
\end{quote}
%

% \begin{theorem}\label{thm:prob}
%   \[\lim_{n \to \infty} \prob{\M(n,R,c,p) \text{ has a solution}} =
%   \begin{cases}
% 1 \text{ if } c > p\\
% 0 \text{ if } c < p
%   \end{cases}\]
% \end{theorem}

Let $N_C$ denote the set of nodes of a knapsack instance that satisfy the capacity constraint and let $N_P$ denote the set of nodes that satisfy the profit constraint.
%%
A solution to the instance exists \emph{if and only if} $N_C\cap N_P \neq \emptyset$.
%
We first consider the capacity constraint and characterise the expected number of nodes that satisfy it, that is, we  characterise the expected cardinality of $N_C$.
%
A set of items $S$ satisfies the capacity constraint if 
{\small\[ \sigma \left( \sum\limits_{i \in S}w_i, \tuple{w_1,\ldots,w_n} \right)  \leq \hat{c} . \]}
That is,
{\small
\[
	\frac{\sum\limits_{i \in S}w_i}{\sum\limits_{i \in I}w_i} \leq   \hat{c},
\]
}
%%
or alternatively,
{\small
\[
	\sum\limits_{i \in S}w_i \leq \ \hat{c}  \sum\limits_{i \in I}w_i.
\]
}

Since the weights are sampled from a probability distribution, we can take expectations on both sides:
{\small
\[
	\ept \left[ \sum\limits_{i \in S}w_i \right] \leq \ept \left[ \hat{c}  \sum\limits_{i \in I}w_i \right].
\]
}
%%
\noindent
Let $\ept[R]$ denote the expectation of $R$. Then
{\small
\[
	\ept \left[ \sum\limits_{i \in S}w_i \right] = k_c\ept[R],
\]
}
%%
\noindent
where $k_c$ is the number of items in $S$ (i.e., the cardinality of $S$).
%%
Similarly,
{\small
\[
	\ept \left[ \sum_{i=1}^{n}w_i \right] = n\ept[R].
\]
}
%%
Since the capacity constraint $\hat{c}$ is fixed and known, we have that $\ept[\hat{c}] = \hat{c}$. Thus, $k_c\ept[R] \leq \hat{c}n\ept[R]$.

Analogous reasoning can be applied to the normalised profit constraint and yields $k_p \geq  \hat{p}n$. A solution to the instance is expected to exist if there exists a $k$ such that $ \hat{c}n\geq k \geq  \hat{p} n $.
%
%Hence, we expect the transition from solvability to insolvability to occur at $\hat{c}/\hat{p}=1$.
Hence, based on Markov's inequality, the condition $\hat{c} < \hat{p}$ is an \emph{upper bound} for the insolvability of instances. 
%

%Hence, for random instances with the property $\hat{c} > \hat{p}$, we expect a knapsack with $k$ items to exists that satisfies both the capacity and the profit constraint.


As a side effect of the analysis above, we can also estimate the number of items in a solution $k$ (if one exists) to a random knapsack instance: \emph{The number of items $k$ in a solution to an instance in $\M(n,R,\hat{c},\hat{p})$ is expected to be between $\hat{c}n$ and $\hat{p}n$ (i.e, $ \hat{c} n\geq k \geq  \hat{p} n $}).
%\todo{I dont get this. the bounds are not tight, so there are many k? how come the expectation has many possibilities?I must be missing something....}

% \begin{corollary}\label{cor:kitems}
%   A solution to an instance in $\M(n,R,c,p)$ is expected to have $k$ items where $ c n\geq k \geq  p n $.
% \end{corollary}

This estimate on the number of items in a solution grounds our intuitive understanding by establishing the solvability conditions for knapsack instances based on the (normalised) capacity and profit constraints. It provides three key insights:
\begin{enumerate}
  \item A knapsack instance is expected to have a solution as long as $\hat{c}\geq \hat{p}$, that is, if the knapsack capacity limit is  higher than the required profit level.

  \item The solutions are expected to be knapsacks with cardinality $k$ (assuming weights and values are drawn from the same distribution). This insight could be useful in developing heuristics for algorithms or to focus the search on specific knapsack configurations.

  \item Normalisation is a useful concept to define parameters that characterise phase transition.
\end{enumerate}

%Based on the above reasoning, we expect a phase transition, that is, a precipitous change from unsolvability to solvability, of knapsack instances to occur when normalised capacity and normalised profit constraints as they approach equality (i.e., $\hat{c}\approx \hat{p}$).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

